Estimating Uniqueness of I-Vector Representation of Human Voice

We study the individuality of the human voice with respect to a widely used feature representation of speech utterances, namely, the i-vector model. As a first step toward this goal, we compare and contrast uniqueness measures proposed for different biometric modalities. Then, we introduce a new uniqueness measure that evaluates the entropy of i-vectors while taking into account speaker level variations. Our measure operates in the discrete feature space and relies on accurate estimation of the distribution of i-vectors. Therefore, i-vectors are quantized while ensuring that both the quantized and original representations yield similar speaker verification performance. Uniqueness estimates are obtained from two newly generated datasets and the public VoxCeleb dataset. The first custom dataset contains more than one and a half million speech samples of 20,741 speakers obtained from TEDx Talks videos. The second one includes over twenty one thousand speech samples from 1,595 actors that are extracted from movie dialogues. Using this data, we analyzed how several factors, such as the number of speakers, number of samples per speaker, sample durations, and diversity of utterances affect uniqueness estimates. Most notably, we determine that the discretization of i-vectors does not cause a reduction in speaker recognition performance. Our results show that the degree of distinctiveness offered by i-vector-based representation may reach 43-70 bits considering 5-second long speech samples; however, under less constrained variations in speech, uniqueness estimates are found to reduce by around 30 bits. We also find that doubling the sample duration increases the distinctiveness of the i-vector representation by around 20 bits.

==> intro_v1.tex <==
Biometric solutions have increasingly become a key component of security systems that govern everyday processes of private and public life. 
%Biometrics solutions are increasing incorporated into everyday devices and processes.
%systems and infrastructures
Today, most smartphones utilize at least one of fingerprint, facial, or iris recognition as the main method for user verification. 
%These an many other physiological biometrics have long been considered a top contender for implementing strong authentication.
Behavioral biometrics are at the core of enterprise information systems to detect anomalies in user interactions and to provide initial as well as continuous authentication.
%static authentication
%such as speech patterns, keystroke dynamics, cognitive biometrics
%The main driver behind this widespread adoption of biometrics for implementing strong authentication and user identification are 
This widespread adoption of biometrics for implementing authentication and user identification is evidently due to 
the fact that biometric traits are unique to the individual, that they are sufficiently invariant, and that they can easily be captured and processed with minimal user intervention. 



%par
Among all types of biometric technologies, there is a more visible growth in the use of voice-based authentication and identification systems. 
%This is partly due to well established expertise in audio signal representation and processing, which continues to further grow by advances in deep learning. 
This is in part due to well-established expertise in audio signal representation and processing \textcolor{black}{and the increase in available computational power in many systems, especially in embedded systems.}
%which substantially improved the achievable system performance.} 
But more importantly, it is due to various application contexts that involve speech-based user interactions where voice as a biometric modality is readily available.
%Beyond that, various application contexts involve speech-based user interaction where voice as a biometric modality is readily available. 
%Beyond that, in some contexts voice as a biometric modality is more readily available
For example, in call center environments verifying the identity of a caller through voice offers a more convenient and cost-effective alternative to conventional knowledge-based authentication where the agent asks the caller a series of questions. 
%In fact, for emerging devices such as wearables that have limited user interface there are only a few alternatives to voice for authentication. 
Moreover, for embedded sensor-enabled devices such as wearables that have limited user interface there are only a few alternatives to voice for authentication.
With the pervasive availability of voice assistants in everyday devices, such as smartphones and IoT devices, 
and the potential integration of voice technology within many applications, speaker verification capabilities will likely become even more important. 
%voice matching and speaker verification capabilities will likely become even more important. 
%voice matching and speaker verification will be of paramount importance.
%of many applications integrating this technology, voice matching and speaker verification will become of paramount importance.
%do voice matching and recognize user's voice. 
%- even predict that nearly every application will integrate voice technology 
%- Speaker verification and ID will also become paramount as part of the voice assistant experience with more security being built around the user.



%par
%\textcolor{black}{Although biometric identifiers are considered to be unique attributes, characterstics, traits

%At its core, the use of a \textcolor{black}{biometric voice representation}, or any other biometric modality for the general case, as part of security systems rests on the uniqueness and individuality of such biometric data. 
At its core, the use of a \textcolor{black}{biometric voice representation}, or any other biometric modality for the general case, as part of security systems rests on the uniqueness and individuality of \textcolor{black}{such biometric identifiers, which may refer to both biological and behavioral attributes.} 
%\textcolor{black}{Although biometric identifiers may refer to both unique biological and behavioral attributes, 
\textcolor{black}{However, acquisition of biometric data through a lossy and error-prone process 
%\hl{that can be} influenced by several environmental factors effectively diminishes discernible characteristics, thereby limiting the biometric information content.
and the variability induced by several environmental factors effectively diminishes discernible characteristics, thereby limiting the biometric information content.
The fact that the representation for the captured voice samples of a speaker may not be unique essentially introduces a vulnerability that can be exploited by attackers.}



%new par
%Voice authentication systems typically utilize a voice model ({\em i.e.,} voiceprint) of the user.
%This model could be created in a text dependent or independent manner, and user verification is performed by matching the voiceprint extracted from a short utterance to a more reliable voiceprint created during the enrollment phase. 
\textcolor{black}{
Voice authentication systems operate by constructing a model of each user's voice. 
With these systems, user verification can be performed in a text dependent or independent manner by evaluating the match of a voice model estimated from test samples to a more reliable model created during user enrollment. 
%Voice authentication systems typically create a model of each user's voice. %which serves as a biometric voice representation. 
%The verification system can be text dependent or independent, and a user is verified by evaluating the match of the voice model estimated from a relatively short utterance to a more reliable model created during user enrollment. 
}
One possible attack against these system\textcolor{black}{s} includes the use of voice synthesis and conversion methods to generate the desired text in a voice that will produce a match with the target speaker, {\em i.e.,} voice-spoofing attacks, 
\cite{ergunay2015vulnerability, turner2019attacking}. %  wu2015sas, wu2016study, wu2016anti}.
\textcolor{black}{No matter how it is performed, such an attack requires access to voice samples of the target user of durations varying from a couple of minutes to several hours \cite{khodabakhsh2017spoofing, baljekar2018speech, Derrick2019}.}
%with durations varying from a couple of minutes to several hours \cite{khodabakhsh2017spoofing, lorenzo2018voice, Derrick2019}.





Since launching such an attack at scale requires a large amount of samples from users, it is not practically feasible \textcolor{black}{most of the time}.  
%A fraudster, however, can alternatively use other speakers’ voice samples to spoof the voice of a target speaker
\textcolor{black}{A fraudster, however, can alternatively use speech samples of other speakers with a similar voice to spoof the voice of a target speaker.}
For this purpose, the attacker can create a dictionary that spans a diverse range of voices, along with sufficient samples, and can quickly identify voice samples most similar to a given query utterance to be used during spoofing.
%For this purpose, the attacker can create a dictionary that spans the space of unique voices and can quickly identify voice samples most similar to a given query voice sample to be used during spoofing.
Unlike many other biometric modalities, it is relatively easy for fraudsters to capture voice for a large population. 
Not only are large numbers of voice samples available online, one can also acquire voice samples by systematically calling phone numbers. 
With robocalling and VoIP technology, such calls can be made at scale at very low cost.
Hence viability of this attack depends largely on the difficulty of creating a voice dictionary of sufficient size to be in the order of unique voice models. 
This ultimately calls for evaluation of the uniqueness of users' voice models, a task which translates into an inquiry into the information content of a biometric modality.
%to the question of determining 
%{\em i.e.,} its size, which can only be determined by evaluating the uniqueness of users' voice models. 
%This ultimately translates to the question of determining the information content of a biometric modality.

%– Voice Synthesis – If the attacker has access to user’s text password (which is same as voice password) and user’s other voice samples, then he/she can perform voice synthesis to gain illegitimate access to the system. Moreover, attacker can also use other user’s voice samples and synthesize the voice sample (the one with higher likelihood) to gain access to the system. The latter is harder but may be feasible when voice features have limited entropy.

%\par
Despite significant research in representation and matching of biometric data, the uniqueness and individuality of biometric modalities have not been studied very thoroughly. 
%This is in fact a relevant problem in a much larger context as biometrics like phenomena associated with embedded hardware, such as imaging sensors \cite{lukas2006digital}, 
%speakers \cite{zhou2014acoustic}, microphones \cite{das2014you}, accelerometers \cite{dey2014accelprint}, gyroscopes \cite{baldini2016experimental}, wireless transceivers \cite{xu2016device} and CPUs \cite{cheng2019demicpu}, are constantly being observed with the assertion that these characteristics \textcolor{black}{can similarly be used for device identification and attribution purposes.}
%can also be used to support similar security functions in the device domain or with respect to their implication for user privacy.
%
%
To date, a number of studies have been undertaken to determine the amount of information contained in a biometric modality including voice, iris, face, and fingerprints. However, measurements provided by different publications vary significantly.
In the case of voice, individuality estimates range between 14 bits \cite{IEEEexample:yang2014} and 120 bits or higher depending on the length of speech samples used for measurements \cite{IEEEexample:entropy2015}. That is, the number of unique human voices is in the order of $2^{14}$ or $2^{120}$. 
Further, a similar pattern has been observed across other modalities, albeit to different extents \cite{sutcu2013biometric}. 
For example, a \textcolor{black}{single} fingerprint, the most mature and well established modality, is estimated to have an entropy of between 12.7 \cite{IEEEexample:takahashi2010} and 55 \cite{young2013entropy} bits.
Similarly, estimates of the uniqueness of biometric face images vary between 12.6 \cite{IEEEexample:takahashi2010} and 55.6 \cite{adler2009towards} bits.
Finally, iris as a biometric modality, which is considered to be the most reliable of all, is estimated to offer 249 \cite{IEEEexample:daugman2003} to 288 \cite{youmaran2012measuring} bits of information.
%is claimed to
Variations up to an order of magnitude (in the exponent) difference in the above estimates indicate the need for a more systematic evaluation.  
%All these variations indicate the need for a more systematic evaluation and approach.
%An order of magnitude difference in estimates in the exponent does not provide a reliable basis to assess the security properties of a voice-biometric system.
%ADD
% flowprint,app fingerprinting from encrypted traffic
% CCS20 EM emanation



%Deconstructing the problem, it is seen that 
%\hl{Three factors play a significant role in variability of the distinctiveness of a biometric modality.}
In fact, three factors play an important role in the discrepancy between reported results on distinctiveness of biometric modalities. 
Biometric data is almost always \textcolor{black}{mapped} into a feature space. 
Hence, an important source of variability is the choice of biometric feature representation. 
Since compact representation of a continuous variable can only be achieved at the expense of information loss, different representations of a biometric modality yield varying  discriminative power. 
The other important factor contributing to difficulty in establishing the uniqueness of a biometric modality is the \textcolor{black}{measurement} of biometric information. 
The inherent variability of a biometric modality combined with the measurement noise and the complexity of modeling high-dimensional feature representations hinder analytical tractability significantly. 
As a result, it becomes difficult to directly utilize the concept of entropy and alternative definitions have been adopted to estimate the inherent entropy.
The last source of variability concerns the dataset used for modeling and measurements. 
Essentially, the accuracy of estimates depends on how well a given dataset reflects the biometric diversity of users and the overall biometric variability exhibited by users. 
However, producing reliable, comprehensive public datasets is a very challenging task due to increasing privacy concerns.
%as it involves revealing part of actual users’s biometric identity. 


%par - backup
%To help close this gap, in this work, we study the problem of measuring the individuality of a biometric modality in the context of voice biometric.
%Our approach to estimation of uniqueness uses known population characteristics as a prior to evaluate the average uncertainty about the identity of a speaker and 
%builds on a mutual information based formulation initially introduced in \cite{tandogan2017towards}.
%Measurements are performed on quantized version of a widely used feature representation in speaker recognition, namely, the i-vector representation. 
%We also study performance implications of operating in a discrete feature domain. 
%In addition, our work brings all approaches to measuring distinctiveness of biometric modalities together and evaluates their strengths and weaknesses from the standpoint of generalizing these measures.


%par
%To help close this gap, in this work, we study the problem of measuring the individuality of a biometric modality in the context of voice biometric.
%Towards this goal, our work brings all approaches to measuring distinctiveness of biometric modalities together and evaluates their strengths and weaknesses from the standpoint of generalizing these measures.
%Our approach to estimation of uniqueness differs from existing ones as it computes the entropy of speaker i-vectors while taking into account within-speaker 
%variability and builds on a mutual information based formulation. 
%Measurements are performed on quantized version of a widely used feature representation in speaker recognition, namely, the i-vector representation.
%Performance implications of operating in a discrete feature domain are also investigated.
%%Most notably, as part of this work, we study the implications of operating in a discrete feature domain on the identification performance. } 
%%We also study implications of operating in a discrete feature domain on speaker recognition performance. 


To help close this gap, in this work, we study the problem of measuring the individuality of a biometric modality in the context of voice biometrics.
Towards this goal, our work brings all approaches to measuring distinctiveness of biometric modalities together and evaluates their strengths and weaknesses from the standpoint of generalizing these measures.
Our approach to estimation of uniqueness differs from existing ones as it computes the entropy of speaker i-vectors while taking into account within-speaker 
variability and builds on a mutual information-based formulation. 
\textcolor{black}{
Measurements are performed on a widely used feature representation in speaker recognition, namely, the i-vector representation.
To be able to estimate the underlying feature distribution as accurately as possible, speaker i-vectors are quantized, %quantized version of features are used, 
and performance implications of operating in a discrete feature space are investigated.
%The level of quantization is determined so that speaker recognition performance yielded by the quantized and the original, non-quantized i-vectors are similar to each other. 
%Further
To ensure that the uniqueness estimates obtained using quantized i-vectors are reflective of the original, non-quantized i-vectors, the speaker verification performances yielded by the two representations are set to similar values.  
}





To evaluate and compare our approach, we created two distinct benchmark datasets in addition to the public VoxCeleb dataset. 
One of these datasets includes voice samples of close to \textcolor{black}{twenty-one} thousand speakers obtained from audio tracks of TEDx Talk videos, and the other
includes samples of 1,595 actors extracted from dialogues in 249 movies.
The former dataset is mainly used to quantify how uniqueness estimates vary depending on number of speakers as well as the amount of speech samples available from each speaker, whereas the latter is used to determine to what degree the true variability intrinsic to a speaker's voice affects estimates.
Overall, the data used in our experiments constitute the most comprehensive set used by a study of similar nature in its effort to better incorporate \textcolor{black}{between}-speaker and within-speaker variability.

%We thus have to deal with variation between speakers, usually known as between-speaker (or inter- speaker) variation
%referred to as

Our paper is organized as follows.
In Section \ref{sec:ses}, we start by reviewing the work done in the field of  speaker recognition and speaker verification with an emphasis on voice models proposed for speaker representation. 
This is followed by a qualitative description of approaches proposed for measuring individuality of a variety of biometric modalities and a discussion of their applicability to voice biometrics in Section \ref{sec:method_entropy}. 
The details of our uniqueness estimation method are given in Section \ref{sec:method}. 
%The two datasets used in experiments along with the process we followed in their creation are described in Section \ref{sec:dataset}.
\textcolor{black}{The datasets used in experiments along with details about the generation of the two new datasets are described in Section \ref{sec:dataset}. }
The \textcolor{black}{evaluation protocol}, results of analyses and uniqueness estimates obtained considering a variety of settings are provided in Section \ref{sec:results}.
We conclude the paper with a discussion of our findings in Section \ref{sec:conclusion}.




==> method_v1.tex <==

The amount of discriminatory information present in a biometric modality has long been a focus of research. 
Early work mainly used the probability of false biometric matching, {\em i.e.} matching a given biometric sample to any other sample by chance for a single user verification attempt, as a measure for estimating individuality \cite{pankanti2002individuality}. 
Setting up a duality with password guessing attacks, O'Gorman \cite{o2003comparing} argued that the sample space of a biometric modality, defined as the valid range of values that can be taken by biometric features, can be used to estimate an upper bound on the individuality of a modality. 
Accordingly, the effective sample space is measured by the inverse of false matching probability which is then mapped to maximal entropy of a modality under the assumption of uniform distribution of sample values. 
In line with this thinking, Dass {\em et al.} \cite{zhu2007statistical} focused on deriving an expression to estimate the probability of a false correspondence between minutiae features of two arbitrary fingerprints. 
This is realized by modeling the distribution of biometric features and using the resulting models to generate random biometric samples needed to calculate the random correspondence probabilities.
%In essence, this approach models the distribution of biometric features and then uses these models to generate random biometric samples needed for calculating random correspondence probabilities.

%Basic idea of this approach is first to estimate a statistical model that explains the distribution of biometric features and then use these models to generate random biometric samples for calculating this probability.

Subsequent approaches to quantifying the amount of information available in different biometric modalities adopted alternative definitions that are more focused on modeling between-subject and within-subject variability of biometric features. 
Below, we provide a brief overview of these approaches, discuss their theoretical underpinnings, and evaluate their applicability to measuring distinguishability offered by the voice as a biometric modality.


%A number of approaches have already been proposed in the context of different of biometric modalities to measure biometric information.
   




\vspace{-0.3cm}
\subsection{\textcolor{black}{Hamming Distance Based Approach}}
In \cite{IEEEexample:daugman2003}, Daugman proposed a method for measuring uniqueness of iris texture and evaluated it on a large collection of iris scans.
The method is based on a feature representation in which each iris scan is transformed into a 2,048-dimensional binary vector (referred to as an iris code) by applying a multi-scale wavelet decomposition to iris textures and encoding the resulting phase characteristics.
%The gist of the estimation method relies on \textcolor{black}{the} comparison of distance based statistics computed from actual user vectors and to those from synthetically generated vectors with elements drawn from a binary distribution in an identically independently distributed (iid) manner.
\textcolor{black}{
The gist of the estimation method relies on \textcolor{black}{the} comparison of pairwise distances measured between actual feature vectors and synthetically generated ones.
The elements of synthetic vectors are drawn from a binary distribution in an \textcolor{black}{independent and identically distributed} (iid) manner to establish a basis for comparison.
}
By interpreting the match between each element of two subject's feature vectors as a Bernoulli trial, the total number of matches is expressed as a random variable. 
%This essentially corresponds to the Hamming distance between the two vectors which is known to follow binomial distribution under the iid assumption. 
This effectively corresponds to the Hamming distance between the two vectors which is known to follow binomial distribution under the iid assumption. 


The binomial distribution can be characterized by the number of elements $N$, the probability of success in each trial $p$, and the variance of the number of matches $\sigma^2$ as
\begin{equation}
\label{eq:daugman}
N = p(1-p)/{\sigma^2}.
\end{equation}
Hence, for an empirically obtained distribution, measured mean and variance values (which are estimators for $p$ and $\sigma^2$) can be used to determine the number of iid elements, $N$, in the vector.
Using this formulation, Daugman computed normalized Hamming distances between iris codes of $4,258$ subjects in a \textcolor{black}{pairwise} manner which yielded more than 9 million comparisons.  
Then, the resulting mean and variance values are evaluated to determine the corresponding degree of freedom in a binomial distribution, {\em i.e.} equivalent $N$ that will yield the same statistic from iid binary vectors, which is found to be 249.
Hence, the binary iris code is estimated to have 249 bits of entropy. 
%Since the iris code is a binary representation, it can be interpreted to have 249 bits of entropy. 


% Tamami repeat edince calisiyor.
% Yarisi repeat edince olmasi gerekenden daha az hesapliyor.
% 200 elemanli vektorun ilk 100 elemeni ikinci 100 ile XOR yapilinca yontem 300 olarak hesapliyor.
% 

This method of estimating uniqueness has certain limitations. 
The reliability of estimation depends on the underlying dependency of the feature vector array. 
Our observations show that for apparent forms of dependencies, such as repetition of the elements in a feature vector, this approach is effective. 
However for more subtle dependencies, say, XOR'ing the first half of the vector with the second half and appending it to the vector, the measured degree of freedom increases proportionally. 
Therefore, the method has a tendency to overestimate the number of independent elements in the vector.

This approach also assumes that each element of the feature vector is equally important as the contribution of each feature to \textcolor{black}{the} Hamming distance is equally weighted. 
Hence, it cannot be generalized to representations where features are sorted \textcolor{black}{according to} their importance. %/representation power. 
In addition, this type of modeling holds only when each element of the feature vector is identically and uniformly distributed. 
Otherwise, the relation given in Eq. (\ref{eq:daugman}) does not hold.  
%and the number of independent elements is overestimated. \hl{neden overestimate ediyor?}
%\hl{Normalized hamming distance ile hesaplanan deger vectordeki elemanlarin olasiliklarin ortalamasi ile hesaplaniyor ve varyans da vectordeki elemanlarin varyanslarinin ortalamalarina denk geliyor. Ama mean linear iken varyans kare(2.dereceden) oldugu icin varyans degeri olmasi gerekenden daha kucuk oluyor ve over estimate ediliyor. Kisaca mean linear, varyans non linear oldugu icin N degeri overestimate ediliyor.(0-1 arasindaki degerlerin karesi daha kuculur.)}
%does not follow the same distribution.
But most critically, since this approach relies on evaluating \textcolor{black}{pairwise} differences between feature vectors, it cannot incorporate within-subject 
%and between-subject 
variations into its formulation. 
In this sense, it is more suitable for biometric modalities where within-subject variability is very limited. 



\vspace{-0.3cm}
%\subsection{\textbf{Relative Entropy of Feature Distributions}}
\subsection{Measuring Relative Entropy in the Feature Space}
An alternative biometric information measurement approach is proposed by Adler {\em et al.} \cite{adler2009towards, IEEEexample:adler2006}  considering facial images and using a relative entropy based formulation.
Relative entropy (also known as Kullback-Leibler divergence) is a non-symmetric measure of the \textcolor{black}{distance between two probability distributions, and it
estimates the average number} of additional bits required to code samples from one distribution when using a code optimized for the other distribution.
%This approach effectively \textcolor{black}{defines} biometric information as the decrease in uncertainty about the identity of a person in the presence of a collection of a set of biometric features that represent population characteristics. 
%This uncertainty is expressed in terms of relative entropy as
This approach effectively \textcolor{black}{defines} biometric information as \textcolor{black}{the additional amount of information needed to describe each individual when 
a collection of biometric features that represent population characteristics are known. 
This is expressed in terms of the relative entropy formulation as}
\begin{equation}
D(p||q) = \int_\mathbf{X} p(\mathbf{X}) \log_2 \frac{p(\mathbf{X})}{q(\mathbf{X})} d\mathbf{X}
\label{eq:RE}
\end{equation}
\textcolor{black}{where $\mathbf{X}$ is a multi-dimensional feature representation, $q(\mathbf{X})$ is the distribution of $\mathbf{X}$ in the overall population, and $p(\mathbf{X})$ denotes the distribution of a subject's features.
%By obtaining empirical distributions of PCA-based statistical features of facial images, 
%average relative entropy between the population distribution and the individual distributions is computed as the measure of biometric information content.}
By assuming multivariate normality for distributions of eigenface features, 
average relative entropy between the population distribution and the individual distributions is computed as an upper bound to biometric information content of face images.
Later, \cite{IEEEexample:entropy2015} applied this approach to voice biometrics considering i-vector feature representation of voice.}
%the average relative entropy between individuals and the population is computed as the measure of biometric information content.

%eigenface method by principal component analysis (PCA) of face images



One limitation of this formulation concerns the fact that modeling within-subject variability requires estimation of too many parameters ({\em e.g.}, mean vector and covariance matrix considering a multivariate normal distribution) which becomes highly error prone when there are only a few samples from each subject.
\textcolor{black}{Therefore, this approach requires deployment of regularization schemes to guard against numerical instability \cite{adler2009towards, IEEEexample:entropy2015}.}
%Further, when actual distributions are not known or are heavy tailed, the estimation becomes less reliable.  
Further, when actual distributions are not normally distributed, the estimation becomes less reliable.  
%Aside from these limitations, this approach has a tendency of overestimating the discrimination entropy as relative entropy provides a measure depending on how a user is different from the population, yet, it does not capture the fact that two users can sufficiently be different from the population but might still be very alike.
%
Aside from modeling and computation difficulties, this definition of biometric information has a tendency to overestimate the \textcolor{black}{level of distinctiveness} as relative entropy provides a measure depending on how a subject is different from the population, yet, it does not capture the fact that two subjects can sufficiently be different from the population but might still be very alike.
%imply how different the two users are from each other.

\vspace{-0.2cm}
%%\subsection{\textbf{Relative Entropy of Matching Score Distributions}}
%\subsection{\textbf{Measuring Information Provided by Verification System in the Score Space}}
\subsection{Measurements in the Matching Score Space}


\textcolor{black}{
Another estimation approach aims at measuring the average information provided by a speaker verification system utilizing matching scores computed by the system.  
In \cite{ramos2008cross}, authors investigated the amount of information needed by a speaker verification system to make a decision as to whether two utterances match. 
Accordingly, the information gain provided by the system is estimated in terms of the cross-entropy between empirical distributions of scores for matching and non-matching speakers and 
the distribution of a variable indicating the prior belief in correctness of a match decision.
% genuine and impostor score distributions
%1. ECE measures the amount of uncertainty (or equivalently, the amount of information required to make a decision) for a likelihood ratio model for a range of priors values.
%2. The ECE can be interpreted as the average information needed to make a decision (between propositions A and B)
%3. The security or evidence level of an automated recognition system can be depicted in terms of the system’s contribution to decision making for forensic or commercial applications, see section 2.4. 
}
%Onemli
%The ECE can be interpreted as the average information needed to make a decision (between propositions A and B) [27, 115]. Thereby, the uncertainty about the propositions is considered (e.g., priors or other knowledge involved in a case).
%
%To simulate information performance over a range of priors,
%To alleviate the limitations of relative entropy based estimation approach due to lack of sufficient user samples needed for modeling, Takahashi {\em et al.} \cite{IEEEexample:takahashi2010} and Sutcu {\em et al.}\cite{sutcu2010measure} independently introduced an alternative approach. 

Later, Takahashi {\em et al.} \cite{IEEEexample:takahashi2010} and Sutcu {\em et al.}\cite{sutcu2010measure} independently introduced an estimation approach to alleviate the limitation of the relative entropy-based measurement approach due to lack of \textcolor{black}{a} sufficient number of subject samples needed for modeling.
%\hl{Another estimation approach} is independently introduced by Takashi {\em et al.} \cite{IEEEexample:takahashi2010} and Sutcu {\em et al.}\cite{sutcu2010measure} to alleviate limitations due to lack of \textcolor{black}{a} sufficient number of subject samples needed for modeling.
%Both approaches are based on the premise that the level of distinguishability provided by a biometric modality not only depends on the utilized feature representation but also on the deployed matching algorithm used for evaluating similarity or closeness between biometric samples, thereby measuring the average biometric information utilized by the overall system.
%To incorporate this into its formulation, \cite{sutcu2010measure} proposed computing the relative entropy between within-user and between-user distributions of the utilized \hl{distance metric} rather than using feature distributions directly. 
\textcolor{black}{To this end, 
\cite{sutcu2010measure} proposed computing the relative entropy between within-subject and between-subject distributions of scores generated by the biometric matching system, rather than using feature distributions directly.}
Alternatively, \cite{IEEEexample:takahashi2010} provided a mutual information based formulation that asymptotically approximates relative entropy in order to obtain the entropy of the biometric system.


%Since this measure relies only on distances, it does not suffer from the difficulty of modeling high-dimensional feature distributions given in Eq. (\ref{eq:RE}). 
%This measure effectively reduces high-dimensional feature distributions given in Eq. (\ref{eq:RE}) to single dimensional distance distributions, and therefore it does not suffer from
%difficulties of estimating parameters of multivariate distributions.
Since these measures \textcolor{black}{only rely on} score distributions, they effectively reduce high-dimensional feature distributions given in Eq. (\ref{eq:RE}) to single dimensional score distributions.
Hence, they do not suffer from difficulties of estimating parameters of multivariate distributions.
In addition, within-subject variability can be captured more accurately as the number of data points needed for modeling increases in proportion to the square of the available number of samples due to pairwise comparison of subject samples. 
%Overall, these resulted with an analytically more tractable approach, and the reliability of estimates depends most critically on accuracy of distribution models.
Overall, this resulted in a more tractable measure where the reliability of estimates mainly \textcolor{black}{depends} on accuracy of the two distributions.
The obvious shortcoming of this type of approach is that it is not a true measure of biometric information content as it also depends on the matching algorithm used for evaluating similarity or closeness between biometric features. 
%\hl{system parameters}.
However, achievable distinguishability within the confines of a biometric identification system is also a key consideration in practical settings. 
%given the specifics of the system it is a viable approach.  



\vspace{-0.3cm}
\subsection{Applicability of Existing Measures to Voice Biometrics}

To determine the \textcolor{red}{uniqueness of a feature representation of speech}, limitations and strengths of these measurement approaches must be evaluated in the context of established feature representation for voice.   
In this regard, an important attribute of i-vectors is that their elements can be assumed independent
because the total variability matrix involved in their calculation can be regarded as an eigenspace with i-vectors functioning as eigenvectors 
%The total variability matrix, $T$, involved in their calculation can be regarded as an eigenspace with i-vectors functioning as eigenvectors.
\textcolor{black}{and further because i-vector elements are decorrelated using a whitening transformation and length normalization \cite{garcia2011analysis}.}
%is centered, whitened, and length-normalized
%This is also confirmed by the covariance matrix of i-vectors being close to diagonal. 
Another attribute concerns the fact that i-vector elements are sorted based on their ability to distinguish speakers as they are obtained through linear discriminant analysis. 
As a result of this, error rates of speaker verification systems do not decrease linearly with decreasing dimensionality of i-vectors.
Lastly, elements of i-vectors are continuous valued and are modeled as a Gaussian mixture distribution as part of the GPLDA based matching process. 
%lenght normalized ---> ...

%\hl{Voice model sectioninda geciyor normalde. Unutmayalim diye burasi sari olarak durmaya devam etsin.}


Considering the overall characteristics of i-vector representation, 
these measures have some shortcomings with respect to their applicability to assess \textcolor{red}{their uniqueness}.
%these approaches are not suitable for measuring uniqueness of human voice. 
In the case of Hamming distance based approach \cite{IEEEexample:daugman2003}, not only each i-vector element has a different discriminative power
but also their quantization will not yield the required uniform distribution.
%but also their quantization will not yield a uniform distribution.
Further, i-vectors have relatively high within-speaker variability which cannot be adequately captured by this approach. 
%Although the relative entropy based estimation approach \cite{IEEEexample:adler2006} \cite{adler2009towards} does not require quantization of i-vector elements, it must be noted that its formulation is more sensitive to modeling errors.
Although the relative entropy based estimation approach \cite{IEEEexample:adler2006} \cite{adler2009towards} does not require quantization of i-vector elements, its formulation is more sensitive to modeling errors \textcolor{black}{as distribution of feature vectors at a high-resolution representation cannot be empirically obtained.}
Since computation of Eq. (\ref{eq:RE}) involves division of two distributions, calculations are more prone to errors at distribution tails where values are small and accurate modeling is typically challenging due to the limited number of samples per speaker.
Moreover, i-vector elements follow a Gaussian mixture model which further increases the number of parameters to be correctly determined.
%Finally, the measurement approach utilizing distance distributions between features, \cite{IEEEexample:takahashi2010, sutcu2010measure}, crucially estimates the distinguishability provided by a speaker verification system. 
\textcolor{black}{Finally, the measurement approach utilizing distance or score distributions between biometric features, \cite{IEEEexample:takahashi2010, sutcu2010measure}, crucially estimates the distinguishability with respect to a similarity or distance metric.} 
\textcolor{black}{This approach potentially underestimates the distinguishability intrinsic to the feature representation as it essentially operates on a function of feature vectors.}
% and cannot be generalized to distinguishability intrinsic to actual feature representations.
%distribution of decision scores

Inspired by the mutual information based formulation of Takahashi {\em et al.} \cite{IEEEexample:takahashi2010}, we introduced a new approach for estimating biometric information content of human voice using i-vector representation \cite{tandogan2017towards}.
\textcolor{black}{Most notably, in this approach, each i-vector is viewed as an instance of a discrete multivariate random variable to obtain a more tangible uniqueness measure defined in terms of the number of bits required to represent i-vectors.
%\hl{Discretizing feature vectors allows for more accurate estimation of feature distributions, as opposed to assuming a particular distribution model for features. 
%Further, by directly operating on feature vectors, instead of utilizing scores or distances computed between features, it provides a more general measure of biometric information content.}
By discretizing feature vectors, this approach allows for more accurate estimation of feature distributions instead of assuming a particular distribution model for features. 
Further, since measurements are performed on actual feature vectors, as opposed to utilizing scores or distances computed between features, this measure provides a more accurate reflection of biometric information content. }
%Therefore, it provides a more general measure of biometric information content.
%HENCE ile ilgili R1 yorumu. revised for better clarity
This study further expands on this initial work to investigate the effects of i-vector discretization more systematically and 
%determines how uniqueness estimates vary depending on the number of speakers under a more accurate modeling of within-subject variability.
%\hl{determines how uniqueness estimates vary depending on several factors that affect modeling between-speaker and within-speaker variability.}
to determine how factors critical to modeling of between-speaker and within-speaker variability affect uniqueness estimates.
The details of our approach are discussed in the following section. 

%Most notably, in this approach, i-vector elements are quantized to obtain a more tangible uniqueness measure defined in terms of the \hl{number of bits}.
%Further, this measure utilizes actual feature vectors by modeling their distribution, instead of using distribution of the distance between user samples.
%\textcolor{black}{Hence}, the resulting estimate is less dependent on verification system parameters.  


